Robust Anthropomorphic Robotic Manipulation through Biomimetic Distributed Compliance

The impressive capabilities of humans to robustly perform manipulation relies on compliant interactions, enabled through the structure and materials spatially distributed in our hands. We propose by mimicking this distributed compliance in an anthropomorphic robotic hand, the open-loop manipulation robustness increases and observe the emergence of human-like behaviours. To achieve this, we introduce the ADAPT Hand equipped with tunable compliance throughout the skin, fingers, and the wrist. Through extensive automated pick-and-place tests, we show the grasping robustness closely mirrors an estimated geometric theoretical limit, while `stress-testing' the robot hand to perform 800+ grasps. Finally, 24 items with largely varying geometries are grasped in a constrained environment with a success rate of 93%. We demonstrate the hand-object self-organization behavior underlines this extreme robustness, where the hand automatically exhibits different grasp types depending on object geometries. Furthermore, the robot grasp type mimics a natural human grasp with a direct similarity of 68%.

==> coverletter.tex <==
We are glad to submit our paper 'TITLE' to Science Robotics. 
In this paper, we introduce a novel approach to the design of anthropomorphic hands, where we seek to match the distributed compliance through the skin, fingers, and wrist to that of human hands. 
This distribution of compliance contributes to passive adaptive behavior from the millimeter to 10cm scale, which collectively contributes to an open-loop behavior robust to environmental uncertainty and human-like.
The robustness and performance of this robot design is thoroughly experimentally validated through measurements of force and finger poses at the low level comparing against a rigid robot configuration, and through full hand grasping and pick-and-place experiments. 
Using an automated pick-and-place setup, we perform over 800+ autonomous grasping experiments and can quantify the performance lies within 20\% with respect to geometric limits. 
Most notably, we show how the self-organization between the fingers and objects underlines the robustness at the full hand scale. Whereby the hand exhibits different grasping methods when object geometries are varied (under the same open-loop control signal), directly matching 68\% of a natural human grasp.

Overall, we show by matching the distributed compliance in addition to the kinematics and motion of a human hand, the resultant behaviors are robust to uncertainty in the environment and exhibits human-like grasping through self-organization. 
Given the open-loop actuation, this robustness can be directly attributed to the passive adaptation from the distributed compliance. 
As such, we believe this makes a significant step forwards in advancing the capabilities of robotic manipulation, the means by which we understand that robustness occurs, and impacts future research directions on sensing and control should be performed to leverage and build upon these embodied capabilities. 

